Transformers for End-to-End InfoSec Tasks: A Feasibility Study

In this paper, we assess the viability of transformer models in end-to-end InfoSec settings, in which no intermediate feature representations or processing steps occur outside the model. We implement transformer models for two distinct InfoSec data formats - specifically URLs and PE files - in a novel end-to-end approach, and explore a variety of architectural designs, training regimes, and experimental settings to determine the ingredients necessary for performant detection models. We show that in contrast to conventional transformers trained on more standard NLP-related tasks, our URL transformer model requires a different training approach to reach high performance levels. Specifically, we show that 1) pre-training on a massive corpus of unlabeled URL data for an auto-regressive task does not readily transfer to binary classification of malicious or benign URLs, but 2) that using an auxiliary auto-regressive loss improves performance when training from scratch. We introduce a method for mixed objective optimization, which dynamically balances contributions from both loss terms so that neither one of them dominates. We show that this method yields quantitative evaluation metrics comparable to that of several top-performing benchmark classifiers. Unlike URLs, binary executables contain longer and more distributed sequences of information-rich bytes. To accommodate such lengthy byte sequences, we introduce additional context length into the transformer by providing its self-attention layers with an adaptive span similar to Sukhbaatar et al. We demonstrate that this approach performs comparably to well-established malware detection models on benchmark PE file datasets, but also point out the need for further exploration into model improvements in scalability and compute efficiency.

==> Background_old.tex <==
\section{Background}
\label{sec:background}

\begin{figure*}[ht]
\centering
\subfloat[Next Character Prediction]{\includegraphics[width=0.3\textwidth]{images/next_char_transformer.png}\label{fig:next}}\hfill
\subfloat[Classification Only]{\includegraphics[width=0.3\textwidth]{images/cls_transformer.png}\label{fig:cls}}\hfill
\subfloat[Classification with Auxiliary Loss]{\includegraphics[width=0.3\textwidth]{images/mixed.png}\label{fig:mixed}}
\caption{For a given context window size, transformers utilize padding/masking operations to perform inference over different sequence lengths. Let $M$ be the length of the sequence and $N$ be the size of the context window, where $M \leq N-1$. Let $C_1$ through $C_M$ be the embeddings corresponding to the sequence elements, in this case, characters within a URL. Let CLS be the embedding corresponding to the CLS token (position $M+1$), and let $PAD_1$ through $PAD_{N-M-1}$ be embeddings of padding tokens. Let $H_1$ through $H_N$ be the final hidden states derived from the transformer. A standard \textit{next character prediction} task is shown in  \protect\subref{fig:next}, where the hidden states are each passed through a classifier $CLS_{Next}$, and the softmax outputs correspond to probabilities of the subsequent tokens. \protect\subref{fig:cls} We can also use the output of $H_{M+1}$, passed through a binary classifier to derive a probability that the input sequence is malicious or benign. \protect\subref{fig:mixed} During training, we can use all token outputs to fit a malicious/benign predictor and a next-character prediction loss simultaneously. Note that hidden states corresponding to padding are ignored. For our implementation, L-R masking operations prevent prior hidden states from attending to any padding-related sequence information.}
\label{fig:transfomer}
\end{figure*}


ML for InfoSec has been researched for decades \cite{rudd2016survey}, but widespread industry adoption has occurred only over the past several years. Of the adopted models, the majority of them utilize some form of hand-crafted features (e.g., \cite{rudd2018meade,rudd2019aloha,anderson2018ember,raff2019kilograms,kyadige2019learning,ducau2019smart}), with only a few operating on raw data. Sequence models, e.g., recurrent neural networks (RNNs) have been applied with some success \cite{pascanu2015malware}, but only to niche problems. Training RNNs for most problems is fundamentally not scalable to long sequences, both in terms of the incremental training times and in terms of lack of the general loss of information from long term dependencies.


Transformers, introduced by Vaswani et al. in \cite{vaswani2017attention} have revolutionized natural language processsing (NLP) and a variety of other discrete sequence modeling domains. This is partly due to their ability to directly incorporate long-term dependencies in a sequence and partly because they are easily trained in parallel. Transformers were originally formulated for sequence transduction tasks, e.g., neural machine translation (NMT), wherein a source sequence is encoded via an encoder stack of attention and feed-forward layers, then decoded via a similar decoder stack, using the input sequence as a source context for decoding to the target sequence. E.g., in an English to French translation model, the encoding of the English sentence would serve as context for the French translated sentence; during translation, the context encoding along with hidden states from the translated portion of the sentence are used to arrive at the next token value. Later models, which constitute massively pre-trained representations, meant for fine-tuning for non-transductive tasks abandon the encoder/decoder setup entirely, opting in favor of either an encoder or a decoder. 


Bidirectional models, e.g., BERT\cite{devlin2018bert}, leverage masked language modeling pre-training to arrive at an encoder whose hidden states can be used for a variety of NLP fine tuning tasks. OpenAI's GPT \cite{radford2018improving} series of models apply a similar approach, but leverage left to right (L-R) masked modeling, in a next-token prediction training regime, wherein a decoder is used to predict subsequent elements of the sequence from previously decoded tokens. A wide variety of modifications to transformers have been made as well, including modeling over multiple modalities and memory/processing optimization tricks to extend context windows to longer lengths, e.g., \cite{lu2019vilbert,sukhbaatar2019adaptive,beltagy2020longformer,kitaev2020reformer,dai2019transformer}. The latter approaches could be interesting when applying transformers to other InfoSec problems/data formats where longer sequences are typical, e.g., classifying malware/benignware from raw bytes of a PE file. In this work, however, we work with relatively short sequences and examine fundamental transformer modeling approaches for a typical InfoSec task.


In contrast to NLP problems where massive corpora are available for pre-training a generic representation, but potentially few labeled examples are available for fine-tuning to a task of interest, many InfoSec applications where ML works well have millions to hundreds of millions of labeled samples. These labels are typically derived from an aggregation of multiple weak labeling sources \cite{ratner2017snorkel,rudd2018meade,fu2020fast}. 
We are not the first to apply transformers to InfoSec tasks.


Li et al. applied transformers to malware detection in \cite{li2019mad}. However, contrary to their approach which is a hierarchical system with multiple transformers trained with multiple different training/fine-tuning regimes, our approach is built on a single end-to-end transformer. While their work is interesting, their evaluation is severely limited in scale ($\sim$ 10k samples) and further evaluation is needed to assess its efficacy in realistic scenarios.


Intriguingly, transformers are amenable to multi-target training, and those that perform next character prediction do so implicitly. Our balanced training methodology, however, is a \textit{multi-task} approach \cite{rudd2016moon}. Several works \cite{rudd2019aloha,ducau2019automatic,huang2016mtnet} have shown that similar multi-task optimization improves the performance of ML on InfoSec tasks. In contrast to these previous approaches, however, it uses a novel technique for re-weighting the per-task loss, such that no auxiliary loss term ever dominates regardless of the loss magnitude.


Our work is not the first to address malicious URL detection -- there are several approaches in the literature that use convolutional architectures to classify malicious/benign URLs and DGA-generated domains including \cite{sahoo2017malicious,saxe2017expose,le2018urlnet,yu2018character}. While these works are interesting, note that they use different benchmark data sets, and are thus not directly comparable to our work. We benchmark against similar convolutional and non-convolutional architectures in this paper, which we have developed internally. Note that the primary focus of this work is not creating the optimal URL classifier, but exploring how to train transformers for a typical non-NLP InfoSec machine learning task and contrasting with transformer training regimes for NLP problems.


While transformers can be implemented in a variety of ways, a typical implementation of a transformer attention stack consists of the following components: 

\begin{enumerate}
    \item Embedding: The input, in our case a URL, is projected into an embedding space. 
    \item Positional Encoding: This is a signal added to each of the embedding vectors to imbue each embedding with a positional order in the sequence (which would otherwise not be tracked by the attention mechanism). This can optionally be added to hidden states within the transformer, but we do not do this.
    \item Multi-Headed Attention Layers: These apply the attention mechanism in parallel in a redundant fashion across $h$ heads. The results are concatenated and fed to a feed-forward layer.
    \item Feed-Forward Layers: These act on each of the hidden states produced by multi-headed attention.
    \item Residual Connections: These add and norm operation between inputs to each stack of attention/FFNN layers. This allows information to percolate up the network and bypass the attention/FFNN blocks when appropriate.
    \item Masks: Because transformers operate in parallel, padding is typically added to inputs shorter than the context window of the transformer. In order to avoid ``attending" to the padding, masking is used. Masking is also used to enforce sequential dependencies, e.g.,  for our implementation, we enforce an L-R sequential dependence.
\end{enumerate}

We will elaborate on the architecture of our specific implementation later on in this paper. However, we present a high-level schematic of how multiple prediction tasks can be performed using a transformer in Fig. \ref{fig:transfomer}. Fig. \ref{fig:next} depicts a standard next-character prediction task from the literature. In this case, the outputs are softmax probabilities over the vocabulary. Fig. \ref{fig:cls} depicts using the transformer as a binary malicious/benign classifier -- the baseline ``decode-to-label" approach presented in Sec. \ref{sec:baseline}. Fig. \ref{fig:mixed} depicts the mixed objective approach presented in Sec. \ref{sec:mixed}, where a loss over the next character prediction output is used as an auxiliary loss in conjunction with the main classification task loss during training.

==> Conclusion_back.tex <==
\section{Conclusion}

We have demonstrated first steps for training transformers from scratch and applying them to an InfoSec dataset. While our URL dataset is not representative of all data in the InfoSec space, it does reflect the common property of having a multitude of samples with labels derived from weak labeling sources, differing from common NLP classification tasks. We have shown that for our use case, unlike in NLP domains, there is little benefit to pre-training, but substantial benefit from mixed objective optimization. We have introduced a novel loss function which dynamically re-balances gradients of auxiliary losses with the main task loss at each training step, potentially improving training stability. We are currently working to extend our models to other data formats, including formats which contain long sequences of generic bytes, to the tune of 1MB. This involves using some of the latest research in extended context sequence length. We are also investigating the use of bidirectional models with different training regimes.

==> Introduction_back.tex <==
\section{Introduction}

The abundance of labeled data %scaling of semi-supervised data labeling 
sources has been a major driver in the success of ML in applications across the board, starting with computer vision, and spreading to many other domains, including InfoSec. However, applications of ML to InfoSec often deal with unique data formats which must be approached differently. This is one of the reasons why, unlike computer vision, NLP, and audio applications to name a few -- which have also seen similar performance improvements and larger labeled data sets -- InfoSec applications of ML still rely heavily on relatively simple models fit on hand-tuned features.

This may be in part because properly learning features based on raw data is less trivial for some of the data formats inherent to security problems, for example, in \cite{anderson2018ember}, MalConv – a convolutional neural network which operates on raw PE files and is closely analogous to vision or NLP convnets \cite{raff2018malware} -- underperforms a lightGBM model trained with default parameters on hand-engineered features. 

Intuition suggests that hand-engineered features potentially leave substantial performance on the table. Given a suitable optimization technique a model capable of operating on raw data can derive its own features that are well-optimized for the task at hand. Moreover, employing such a model allows for a simpler train/deploy pipeline across different formats. Thus there is an impetus for research into more effective ML models for InfoSec tasks that operate on raw data.



With respect to other domains where ML models operating on raw data have advanced the state of the art, natural language processing (NLP) is arguably most analogous to InfoSec tasks. Some InfoSec tasks can even be framed as NLP problems, including email spam detection \cite{dada2019machine}, website content categorization \cite{rao2019detection}, social media disinformation triage \cite{seymour2016weaponizing}, and certain areas of data leak prevention (DLP) \cite{alzhrani2016automated,alzhrani2016automated2,alzhrani2017automated}. Other InfoSec tasks, which cannot directly be framed as NLP problems still face similar challenges, for example, these tasks typically contain long-ranging sequential dependencies, where, at inference, one or more tokens that are far-removed from a given token in the sequence may strongly influence the probability of that token. Given the close analogy to NLP and because transformer architectures have revolutionized performance in the NLP domain, it seems fruitful to explore the feasibility of applying transformers to InfoSec tasks, especially since they somewhat address the long range dependency issue. 

However, InfoSec is a broad field, and sequential dependency ranges vary dramatically based on the data type.  In NLP literature, “long-range” dependencies are typically 
considered to span tens to tens of thousands of tokens – often backwards -- within a sequence. While similar ranges may apply for certain types of InfoSec tasks – e.g., infosec tasks that are built on natural language – for other tasks -- e.g., binary classification where function calls and declarations can be almost arbitrarily separated -- relevant dependencies can span forward or backward millions or even billions of bytes.

While some research has been conducted on scaling transformer context window sizes and additional research is required to develop transformer architectures for other InfoSec tasks, in this paper, we perform an initial feasibility study in which we train transformers to detect malicious URLs. Malicious URL detection has the advantage that it is an InfoSec task which cannot be framed directly as an NLP problem, yet the relatively short sequence lengths fit into transformers' context windows without introducing additional modifications for longer sequences (e.g., hidden state caching, sparse attention patterns, locality sensitive hashing, etc.). 

Malicious/benign URL data/classification also has certain characteristics which, to a point, resemble those of other InfoSec datasets/problems: Contrary to NLP tasks, where large datasets are available for pre-training, but relatively small datasets are available for fine tuning, many InfoSec classifiers are fit on large quantities of weakly labeled data, labeled, e.g., by aggregating over threat feeds or externally derived vendor scores. Thus, this feasibility study provides some preliminary insight on how best to train transformer architectures in this problem setting. Contemporaneous work on scaling transformer context windows for different InfoSec data formats, we defer to another paper. The contributions of this paper are as follows:

%This paper constitutes a preliminary exploration of this question, using a dataset of malicious and benign URLs. This allows us to work with large quantities of relevant data that reflect a typical InfoSec use case, yet contain short enough sequences to apply fundamental transformer architectures. Contemporaneous work on scaling transformer context windows for different data formats, we defer to another paper. The contributions of this paper are as follows:

\begin{itemize}
    
    \item A performance comparison between our novel transformer approaches and other more conventional approaches to URL classification. Using a transformer model, we are able to achieve performance on par with our top benchmark models.
    
    \item A performance comparison of multiple URL transformer training regimes, including with and without auto-regressive pre-training. We demonstrate that in contrast to NLP applications which rely heavily on unsupervised pre-training, this strategy does not readily improve performance on the URL classification task.
    
    \item A novel balanced mixed objective transformer loss function which balances a classification objective with an auxiliary auto-regressive objective during training.
    
 \end{itemize}



%Data for these types of tasks have their own unique considerations. Contrary to NLP, where large datasets are available for pre-training, but relatively small datasets are available for fine tuning, InfoSec classification tasks typically contain large quantities of weakly labeled data, labeled, e.g., by aggregating over threat feeds or externally derived vendor scores. Thus, it is a very open question how best to train transformer architectures for these types of problems. 


% Data for InfoSec tasks typically contains long-range sequential dependencies -- e.g., a function call later in a file might be referenced in a header, the structure of a file system at a given domain will depend on that domain, etc. In close analogy to NLP tasks, where transformer models, introduced in \cite{vaswani2017attention} have attained state-of-the-art performance precisely by explicitly incorporating long-term dependencies into their predictions, we propose to use transformers for generic InfoSec tasks. There are some InfoSec tasks that are built directly on top of natural language processing -- tasks like email spam detection \cite{dada2019machine}, website content categorization \cite{rao2019detection}, social media disinformation triage \cite{seymour2016weaponizing}, and certain areas of data leak prevention (DLP) \cite{alzhrani2016automated,alzhrani2016automated2,alzhrani2017automated} to name a few. For these tasks, it is easy to fine-tune NLP transformers using standard NLP pipelines. However, to the best of our knowledge, transformers have not been trained end-to-end, from scratch, for generic ML security tasks. Other information security tasks that are not NLP-based, use different types of data that are highly sequential, but cannot necessarily leverage stock NLP models. These include malware/benignware classification and categorization, code authorship attribution, and classification of URLs, filepaths, and registry keys to name a few. In order to apply transformer architectures to these tasks, models must be trained from scratch. 

% Given the long-ranging sequential dependencies present in samples for a variety of security tasks, and given a degree of analogy with certain NLP tasks, transformers seem like natural candidates. While fine-tuned NLP transformers have previously been applied to security task that are built on natural language processing  -- tasks like email spam detection, website content categorization, social media disinformation triage, and certain areas of data leak prevention (DLP) to name a few -- transformers have not been trained from scratch for end-to-end ML security tasks. 

% Data for these types of tasks have their own unique considerations. Contrary to NLP, where large datasets are available for pre-training, but relatively small datasets are available for fine tuning, InfoSec classification tasks typically contain large quantities of weakly labeled data, labeled, e.g., by aggregating over threat feeds or externally derived vendor scores. Thus, it is a very open question how best to train transformer architectures for these types of problems. 




%While there are a variety of different ML-Sec problems/data formats for ML-Sec problems, 


%The scaling of semi-supervised data labeling sources, largely thanks to vendor aggregation services, has revolutionized the security industry to the point where relatively rudimentary ML models complement, and in some respects outperform signature-based approaches. This is in large part due to sheer training data scale, where even simple feed-forward neural networks fit on low SNR features are capable of delivering state-of-the-art detection performance.  Given that the industry now possesses data at scales thought be unfathomable a few years back, a logical question arises: why are so many antimalware vendors using such naïve ML models in their detection technology?

%Many of the models discussed in recent literature are far from “powerful” by today’s standards \todo{Need references to back this up}. For example, OpenAI’s GPT-3 transformer consists of 175-billion parameters, six to seven orders of magnitude more parameters than models typically trained from scratch for security-related tasks – though there have been several attempts to fine-tune NLP models for security tasks. While for endpoint applications which must be highly resource cognizant, ML model sizes are inherently limited, Security as a Service (SaaS) and Intelligence as a Service (IaaS) applications can accommodate much larger model sizes, because these ML models can reside on dedicated servers with custom hardware configurations and most SaaS and IaaS applications are not quite so latency-sensitive. 

%While training GPT-3 scale models might be beyond the scope of most security vendors’ compute resources – indeed models must also be retrained/fine-tuned on a regular basis to address concept drift, most security vendors still have the infrastructure to use far more powerful models than they currently do, and will -- increasingly so -- as technology advances into the 2020s. Moreover, data scales will continue to grow and there is also the very real likelihood that the performance of low-SNR features will saturate. 

% \todo{Teaser Diagram}

% We argue that it is vital that the security industry keep up with and advance the state of the art in ML modeling, adapting novel, powerful, ML architectures, to our industry’s unique data sources and modalities. This means utilizing the latest in sequence modeling, including models, which support long-range dependencies, that are variable in length, and can be trained over large datasets in a scalable and parallel manner. 

% Some information security tasks, which leverage natural language data are inherently NLP tasks, which can leverage fine-tuned transformers, pre-trained at large scale. These include email spam detection, website content categorization, social media disinformation triage, and certain areas of data leak prevention (DLP) to name a few.


% Other information security tasks, however, use different types of data that are highly sequential, but cannot necessarily leverage stock NLP models. These include malware/benignware classification and categorization, code authorship attribution, and classification of URLs, filepaths, and registry keys to name a  web few. In order to apply transformer architectures to these tasks, models must be trained from scratch. 


% Data for these types of tasks have their own unique considerations. Contrary to NLP, where large datasets are available for pre-training, but relatively small datasets are available for fine tuning, InfoSec classification tasks typically contain large quantities of weakly labeled data, labeled, e.g., by semi-supervised threat feeds or external vendor aggregation services. Thus, it is a very open question how best to train transformer architectures for these types of problems. 

% This paper constitutes a preliminary exploration of this question, using a dataset of malicious and benign URLs. This allows us to work with large quantities of relevant data that reflect a typical InfoSec use case, yet contain short enough sequences to apply fundamental transformer architectures. Contemporaneous work on scaling transformer context windows for different data modalities, we defer to another paper. The contributions of this research are as follows:

% \begin{itemize}
%     \item A performance comparison between our novel transformer approaches and other more conventional approaches to URL classification.
%     \item A performance comparison of multiple transformer training regimes, including with and without pre-training.
%     \item A novel balanced mixed objective transformer loss function.
%  \end{itemize}
